A Case Study in Astronomical 3-D Printing: The Mysterious Eta Carinae

3-D printing moves beyond interactive 3-D graphics and provides an excellent tool for both visual and tactile learners, since 3-D printing can now easily communicate complex geometries and full color information. Some limitations of interactive 3-D graphics are also alleviated by 3-D printable models, including issues of limited software support, portability, accessibility, and sustainability. We describe the motivations, methods, and results of our work on using 3-D printing (1) to visualize and understand the Eta Car Homunculus nebula and central binary system and (2) for astronomy outreach and education, specifically, with visually impaired students. One new result we present is the ability to 3-D print full-color models of Eta Car's colliding stellar winds. We also demonstrate how 3-D printing has helped us communicate our improved understanding of the detailed structure of Eta Car's Homunculus nebula and central binary colliding stellar winds, and their links to each other. Attached to this article are full-color 3-D printable files of both a red-blue Homunculus model and the Eta Car colliding stellar winds at orbital phase 1.045. 3-D printing could prove to be vital to how astronomer's reach out and share their work with each other, the public, and new audiences.

==> views_ApastronHighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={ApastronHighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={ApastronHighMdotWWCR}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronHighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWIR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronHighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={ApastronHighMdotBase}
    VISIBLE=false
  END
END


==> views_PeriastronHighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={PeriastronHighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={PeriastronHighMdotWWCR}
    VISIBLE=true
  END
  PART={HighMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronHighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWIR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronHighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={PeriastronHighMdotBase}
    VISIBLE=false
  END
END


==> views_Phase1p045HighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={Phase1p045HighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={Phase1p045HighMdotWWCR}
    VISIBLE=true
  END
   PART={HighMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045HighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWIR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045HighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={Phase1p045HighMdotBase}
    VISIBLE=false
  END
END


==> views_color.tex <==
VIEW={Joined}
  COO=16.551864624023438 -22.931995391845703 31.491222381591797
  C2C=-0.7463229298591614 0.18275338411331177 0.6400026082992554
  ROO=22.455231612205928
  ROLL=-0.8744158653055476
  AAC=60.000001669652114
  %BGCOLOR=0.784314 0.784314 0.784314
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={WWIR}
    VISIBLE=true
  END
    PART={PrimaryWind}
    VISIBLE=true
  END
   PART={Stars}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=16.551864624023438 -22.931995391845703 31.491222381591797
  C2C=-0.7463229298591614 0.18275338411331177 0.6400026082992554
  ROO=22.455231612205928
  ROLL=-0.8744158653055476
  AAC=60.000001669652114
  %BGCOLOR=0.784314 0.784314 0.784314
   BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={WWIR}
    VISIBLE=false
  END
END
VIEW={WWIR}
  COO=16.551864624023438 -22.931995391845703 31.491222381591797
  C2C=-0.7463229298591614 0.18275338411331177 0.6400026082992554
  ROO=22.455231612205928
  ROLL=-0.8744158653055476
  AAC=60.000001669652114
  %BGCOLOR=0.784314 0.784314 0.784314
   BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PrimaryWind}
    VISIBLE=false
  END
 END

